CodoMo: Python Model Checking to Integrate Agile Verification Process of Computer Vision Systems

Model checking is a fundamental technique for verifying finite state concurrent systems. Traditionally, model designs were initially created to facilitate the application of model checking. This process, representative of Model Driven Development (MDD), involves generating an equivalent code from a given model which is verified before implementation begins. However, this approach is considerably slower compared to agile development methods and lacks flexibility in terms of expandability and refactoring. We have proposed "CodoMo: Python Code to Model Generator for pyModelChecking." This tool automates the transformation of a Python code by an AST static analyzer and a concolic testing tool into intermediate models suitable for verification with pyModelChecking, bridging the gap between traditional model checking and agile methodologies. Additionally, we have implemented a multiprocess approach that integrates the execution of PyExZ3 with the generation of Kripke structures achieving greater work efficiency. By employing CodoMo, we successfully verified a Tello Drone programming with gesture-based image processing interfaces, showcasing the tool's powerful capability to enhance verification processes while maintaining the agility required for today's fast-paced development cycles.

==> deleted_Problem_Setting_Gautam.tex <==
\section{Problem Setting}: Gautam

While significant works regarding model checking and system verification's are reported in the literature, critical open research questions persisted in the domain of unmanned vehicle and flying objects including drones. We argued that traditional model checking methodologies rely on Model Driven Development (MDD), where models are designed first, and code is generated from these models. However, this approach is considerably slower than agile development methods and lacks flexibility in terms of expandability and refactoring. This gap between traditional model checking and agile methodologies limits the effective verification of software models in dynamic and fast-paced development environments. \par
Our challenge is to automate the transformation of Python code into models suitable for verification with PyModelChecker, enabling the efficient verification of agile software projects while bridging the gap between traditional model checking and modern development methodologies. \par
From our literature survey, we identified the following research gaps:
\begin{enumerate}
\item RQ1: How can safety and reliability properties be effectively verified in increasingly connected and autonomous drone-like unmanned flying objects? 
\item RQ2: How can the transformation of Python code into formal models be automated to facilitate model checking with PyModelChecker?
\item RQ3: How can model checking techniques be applied to gesture-based image processing interfaces in Tello Drone programming using CodoMo?
\item RQ4: What are the limitations and challenges of using CodoMo for agile software verification, and how can they be addressed in future work?
\end{enumerate}
